A Local Graph Limits Perspective on Sampling-Based GNNs

We propose a theoretical framework for training Graph Neural Networks (GNNs) on large input graphs via training on small, fixed-size sampled subgraphs. This framework is applicable to a wide range of models, including popular sampling-based GNNs, such as GraphSAGE and FastGCN. Leveraging the theory of graph local limits, we prove that, under mild assumptions, parameters learned from training sampling-based GNNs on small samples of a large input graph are within an $\epsilon$-neighborhood of the outcome of training the same architecture on the whole graph. We derive bounds on the number of samples, the size of the graph, and the training steps required as a function of $\epsilon$. Our results give a novel theoretical understanding for using sampling in training GNNs. They also suggest that by training GNNs on small samples of the input graph, practitioners can identify and select the best models, hyperparameters, and sampling algorithms more efficiently. We empirically illustrate our results on a node classification task on large citation graphs, observing that sampling-based GNNs trained on local subgraphs 12$\times$ smaller than the original graph achieve comparable performance to those trained on the input graph.

==> draft_alg_Apr23.tex <==

\subsection{Sampling-Based GNNs: An Algorithmic Framework}

The demand to scale Graph Neural Networks (GNNs) and handle larger and more complex graphs is increasing as the  graph data sizes continue to grow. At the same time training GNNs on large-scale graphs requires significant computational resources and memory usage. To overcome these challenges, recent research suggests using diverse sampling techniques.


This paper aims to develop a general unified framework for sampling-based GNN architectures. We propose formalizing algorithms that utilize sampling in two different ways. First, nodes are sampled to estimate the gradient and update the weights for the next iteration. We refer to this as \emph{node sampling}. Second, a sampling method is used to prune the computational graph in computing the node embeddings. We refer to this as \emph{computational-graph sampling}. We describe each of these types of sampling next, and then we make a formal abstraction of sampling-based GNNs.

% To provide a more general framework that abstracts away from the details of specific architectures, we formalize a class of algorithms based on sampling. Sampling is a key technique used in this class of algorithms, typically employed in two steps. First, nodes are sampled to estimate the gradient and update the weights for the next iteration. We refer to this as \emph{node sampling}. Second, a sampling method is used to prune the computational graph in computing the node embeddings. We refer to this as \emph{computational graph sampling}. We describe each of these types of sampling next, and then we make a formal abstraction of sampling-based GNNs.

% Node sampling

\subsubsection{Node sampling for gradient computation}


Due to the difficulty of computing gradient descent on large graphs, stochastic gradient descent (SGD) over graph nodes is commonly utilized. SGD in its vanilla form samples a minibatch of nodes $V_B\subset V(G)$ and then uses the gradient on these nodes to estimate \eqref{eqn:GD}, i.e., it uses $\smash{\frac{1}{|V_B|}\sum_{v\in V_B}\nabla_{\mathbf W}\mathcal L(\mathbf z_v)}$ as an estimator of $\nabla_{\mathbf W}\mathcal L(\mathbf Z)$. 

Variants of SGD use importance sampling for estimating the gradient (for example, in GraphSAINT\cite{zeng2019graphsaint}). Let $\nu_g:G\to\mathbb R^+$ be a weight function determining the probability of sampling as $\smash{\frac{\nu_g(G,v)}{|V(G)|}}$. Then, the following is an estimator for \eqref{eqn:GD},
\begin{equation}\label{eq: loss estimate weighted}
 \nabla_{\mathbf W}\tilde{\mathcal L}_{\nu_g}(\mathbf Z)=\frac{1}{|V_B|}\sum_{v\in V_B}\frac{1}{\nu_g(v)} \nabla_{\mathbf W} \mathcal L(\mathbf z_v).
\end{equation}
In the case of vanilla SGD, $\nu_g(v)=1$ for all $v \in V(G)$.

% Computational graph sampling

\subsubsection{Computational-graph sampling} \label{sbs:comp_sampling}

In GNN-based architectures, a second sampling function called $\nu_C$ is often used to draw the computational graph. When $\nu_C$ is applied to a particular node $v$, it outputs a sampled computational graph denoted by $\nu_C(G,v)$ (or simply $\nu_C(v)$ if $G$ is clear from context). This sampled computational graph contains all the necessary attributes and its size depends on the number of layers in the architecture since it is used to compute the embedding in \eqref{eqn:propagation}. 
With this sampling process established, we can now proceed to examine the algorithm.

\todo{\bf Amin: the above paragraph needs to be rewritten.}
% \red{L: I think we can probably add an equation for the probability of adding a node $u$ to the computational graph of $v$ here, right? Here is a suggestion:
% \begin{equation*}
%     (u,v) \sim \frac{\nu_C(v,u)}{|N(v)|} 
% \end{equation*}
% }

% The algorithm

\subsubsection{The algorithm}\label{sec: alg}
At an abstract level, the classic algorithm for training sampling-based GNNs takes a graph as input, along with a gradient sampler $\nu_g$, a computation graph sampler $\nu_C$, and aggregator functions. This algorithm constructs the GNN model on an entire graph. The algorithm iteratively samples a minibatch of nodes from the entire graph based on $\mu_g$, performs forward and backward propagation on the computational graph using $\nu_C$ (as in \eqref{eqn:propagation}), and then computes loss functions on the sampled nodes. Finally, it updates the weights with gradient descent at each round (see full description in Algorithm~\ref{alg: classic} in the appendix).   It is worth noting that the input graph remains unchanged during the training process.


We propose a slight modification to this algorithm based on the theory of graph limits. Instead of training on the full-sized graph, our algorithm takes a sequence of graphs as input. It visits a new graph at each iteration, builds the computation graph, updates the gradient only on the current graph, and terminates the iteration once the gradient magnitude falls below a certain threshold.

The idea is to give small samples from the original large graph as the input. In the following sections, we will use the theory of graph limits to show that if the input graph sequence has a similar local structure as a large graph, then this modification in training allows for efficiency without significantly changing the original algorithm.



% repeatedly samples mini-batches $V_B\sim\nu_g$ from the current graph, builds a computation graph for the sampled nodes using $\nu_C$, computes embeddings for the sampled nodes with forward propagation, computes the loss on the sampled nodes, and updates the coefficients using backward propagation. The algorithm terminates once the gradient magnitude falls below a certain threshold. This modification allows for more efficient training without significant changes to the original algorithm.

% At an abstract level, the algorithm gets a gradient sampler $\nu_g$, a computation graph sampler $\nu_C$, and aggregator functions as the inputs. Instead of training on the entire graph (which is large), the algorithm takes sequences of graphs of smaller size as input. Then, the algorithm repeatedly samples mini-batches $V_B$ from the current graph, builds a computation graph for the sampled nodes using $\nu_C$, computes predictions for the sampled nodes with forward propagation, computes the loss on the sampled nodes, and updates the coefficients using backward propagation. The algorithm terminates once the gradient magnitude falls below a certain threshold. 

{\bf: Amin:} This is my first major comment. We should rewrite the algorithm. Right now, the algorithm requires a sequence of graphs as   input. Instead, we should make the input one graph. That way,  Algorithm 1  will be the common generalization of the various sampling-based GNNs. 

The first three paragraphs before the description of the algorithm should describe how this framework gives graphsage, fastgcn etc... as special cases. 


\begin{algorithm}[htb!]
   \caption{Sampling-based GNN}
   \label{alg:}
\begin{algorithmic}
   \State {\bfseries Input:} A sequence of graphs $\{G_n\}_{n\in\mathbb N}$, gradient sampler $\nu_g$; computational graph sampler $\nu_C$; aggregator functions $\text{AGGREGATE}_\ell, \text{COMBINE}_\ell$ for $\ell\in\{0,\dots,L\}$; depth $L$.
   \Repeat
   \State Sample minibatch of nodes $V_B$ from  $V(G_t)$ proportional to weights $\nu_g$.
   \For{$v\in V_B$}
   \State Sample the computation graph $G_v$ with respect to distribution $\nu_C(v)$
   \For{$\ell =0$ to $L$}
   \State $\mathbf{h}^{(\ell+1)}_{N(v)}=\text{AGGREGATE}_\ell(\{\mathbf h^{(\ell)}_u,(u,v)\in E(G_v)\}$
\State $\mathbf h^{(\ell+1)}_v =  \text{COMBINE}_\ell\Big(\mathbf{h}^{(\ell+1)}_{N(v)}, \mathbf{h}^{(\ell+1)}_{v}\Big)$
\EndFor
\State $\mathbf z_v=\mathbf h^{(L)}_v$
   \EndFor
   \State $\nabla_{\mathbf W_t}\tilde{\mathcal L}_{\nu_g}(\mathbf Z)=\frac{1}{|V_B|}\sum_{v\in V_B}\frac{1}{\nu_g(v)} \nabla \mathcal L(\mathbf z_v).$
   \State    $\mathbf{W}_{t+1}=\mathbf{W}_t-\eta \nabla_{\mathbf W_t} \nabla\tilde{\mathcal L}_{\nu_g}$
   \State $t\leftarrow t+1$
   \Until{$|\nabla\mathcal L|\leq\epsilon$}
\end{algorithmic}
\end{algorithm}

As we will discuss in detail in Section~\ref{sec: convergence result}, many architectures such as GraphSAGE, FastGCN, GraphSAINT, and ShaDoWGNN fit into the description of this algorithm.


==> full_gcn.tex <==
\section{Proof of Theorem~\ref{thm: GCN}}
We begin the proof by relating the gradient of loss function on finite samples to the gradient of the loss function in the limit.
To formalize the proof, let $\mathcal L(W_t,G)$  be the loss of applying $W_t$ (coefficients at iteration $t$ of the algorithm) to graph $G$ \footnote{ For simplicity, we don't show the input feature in this representation. But all results apply to convergent graphs with input features.}. 
\begin{lemma}\label{lm: nabla bound}
Given assumptions of Theorem~\ref{thm: GCN}, for any given $t>0$,
\[\nabla\mathcal L(W_t,G_n)\overset{\mathbb P}{\to} \mathbb E_\mu[\nabla\loss(W_t,G)]\]
% \begin{align*}
%     \lim_{n\to \infty}\mathbb P\Big(|\nabla\mathcal L(W_t,G_n)-\mathbb  E_\mu[\nabla\mathcal L(W_t,G)]|\\
%     \qquad\qquad \leq \frac{1}{2}\mathbb E_\mu[\nabla\mathcal L(W_t,G)]\Big)=1,
% \end{align*}
where the probability is over the possible randomness of $G_n$.
\end{lemma}
\begin{proof}
Proof sketch: Since $f$ is almost local and that the computation graph depends on $K$ layers,  then the loss is a local function. Given that the activation function is Lipschitz, then the loss is continuous and bounded as well. 
Then the convergence to limit follows from the definition of local limits.
\end{proof}


Using this bound, we will show that the loss decreases in the limit as the number of sampled graphs increases.

 
\begin{lemma}\label{lm: decay in loss}
Given the assumption of Theorem~\ref{thm: GCN}, fix some $\epsilon>0$. Also assume the learning rate $\eta$ is smaller than $1/C$, where $C$ is the loss function's Lipschitz constant.
Then there exists some $N_\epsilon$ such that if  Algorithm~\ref{alg: GCN} is trained on graphs of size larger than $N_\epsilon$, then
the loss on the limiting graph decreases in  each iteration,
\begin{align*}
\mathbb P\Big(\mathbb E_\mu[\loss(W_{t+1},G)]\leq\\ \mathbb E_\mu[\loss (W_t,G)]-\frac{\eta}{4}||\mathbb E_\mu[\nabla\loss(W_t,G)]||^2\Big)\geq 1-\epsilon,
\end{align*}
where the probability is over the sampled graph $G_n$ in iteration $t$.
\end{lemma}
\begin{proof}
We use a helper function to smooth out the difference  between the two steps of the loss function. 
Let (in the following the expectation is over the limit $G$),
\[g(\epsilon)=\mathbb E_\mu[\mathcal L(W_{t}-\epsilon\eta \nabla\mathcal L(W_t, G_n), G))].\]
Then $g(1)=\mathbb E[\loss(W_{t+1},G)]$ and $g(0)=\mathbb E[\loss(W_{t},G)]$.
Then $\frac{\partial g}{\partial \epsilon}=-\eta \nabla\mathcal L(W_{t},G_n) \mathbb E_\mu[\nabla\mathcal L(W_{t}-\epsilon\eta \mathcal L(W_{t},G_n), G))].$
Then 
\begin{align*}
    g(1)-g(0)&=\int_0^1\frac{\partial g}{\partial \epsilon }d\epsilon.\\
    &=-\eta \nabla\mathcal L(W_{t},G_n)\\
    &\int_0^1\mathbb E_\mu[\nabla\mathcal L(W_{t}-\epsilon\eta \mathcal L(W_{t},G_n), G))]d\epsilon
\end{align*}
Then we add and subtract $\mathbb{E}_\mu[\nabla\loss(W_{t},G)]$ to get
\begin{align*}
  & \loss(W_{t+1},G)-\loss(W_{t},G)\\
  &  =-\eta \nabla\mathcal L(W_{t},G_n)\mathbb E[\nabla\loss(W_{t},G)]\\
  &  +\eta\nabla\mathcal L(W_{t},G_n)\Big( \int_0^1\nabla \mathcal L(W_{t}
  -\epsilon\eta \nabla\mathcal L(W_t,G_n), G)\\&-\mathbb E_\mu[\nabla\mathcal L(W_t, G)]d\epsilon\Big)
\end{align*}
Now since $\nabla \mathcal L$ is Lipschitz (with constant $C$),
% Then by applying Lemma~\ref{lm: nabla bound},
\begin{align*}
  &   \loss(W_{t+1},G)-\loss(W_{t},G)\\
  &  \leq -\eta \nabla\mathcal L(W_{t},G_n)\mathbb E[\nabla\loss(W_{t},G)]\\
  &  +\eta| \nabla\mathcal L(W_{t},G_n)|\Big( \int_0^1\epsilon\eta C||\nabla\mathcal L(W_t, G_n)||d\epsilon\Big)\\
  &=-\eta \nabla\mathcal L(W_{t},G_n)\mathbb E[\nabla\loss(W_{t},G)]+\frac{\eta^2 C}{2}||\nabla\mathcal L(W_t, G_n)||^2\\
  &=\frac{\eta^2 C-\eta}{2}||\nabla\mathcal L(W_t, G_n)||^2\\
 & \qquad-\frac{\eta}{2}\Big(||\mathbb E_\mu[\nabla\loss(W_{t},G)]||^2-||\nabla\mathcal L(W_t, G_n)\\
 &\qquad-\mathbb E_\mu[\nabla\loss(W_{t},G)]||^2\Big)
\end{align*}
We can bound the first term by choosing the learning rate $\eta$ smaller than $1/C$, and the second term by using Lemma~\ref{lm: nabla bound}.
\end{proof}


Now, we are ready to prove the theorem.
We use the last result together with Lemma~\ref{lm: nabla bound} to upper bound the number of steps that it takes for the  algorithm to converge. 
\begin{proof}
Given  $\epsilon>0$ define the stopping time 
\[t^*=\inf_t\{\mathbf{E}_{\mu,W_t}(\nabla \loss(W_t,G))\leq \epsilon\},\]
where the expectation is both over the randomness of the limit $G$ and the coefficients $W_t$, where the randomness of $W_t$ is due to the randomness of sampling the graph $G_n$. %\red{(L: Why is the expectation also over $W_t$? Is it because of the randomness of $W_0$?).}\blue{Y: no it's because of randomness of $G_n$. }
We write loss as the sum of differences
\begin{align*}
    \mathbf{E}_{\mu,W_t}\big( \loss(W_{0},G)-\loss(W_{t^*},G)\big)=\\
        \mathbf{E}_{\mu,W_t}\big( \sum_{t=0}^{t^*-1}\loss(W_{t},G)-\loss(W_{t+1},G)\big).
\end{align*}
We can take the expected value with respect to the randomness of $t^*$,
\begin{align*}
   \mathbb E_{t^*} \mathbf{E}_{\mu,W_t}\big(\loss(W_{0},G)-\mathcal L(W_{t^*},G)\big)=\\
      \sum_{t^*=0}^{\infty}  \mathbf{E}_{\mu,W_t}\big(     \sum_{t=0}^{t^*-1} \loss(W_{t},G)-\loss(W_{t+1},G)\big)\mathbb P(t^*).
\end{align*}
    By applying Lemma~\ref{lm: decay in loss} for $t<t^*$,
    \[\mathbb P\Big( \mathbf{E}_\mu\big(\loss(W_{t},G)-\loss(W_{t+1},G)\big)\geq \frac{\eta}{4}\epsilon^2\Big)\geq 1-\epsilon.\]
    By applying this to the previous inequalities:
    \begin{align*}
   \mathbb E_{t^*} \mathbf{E}_{\mu,W_t}\big( \loss(W_{0},G)-\loss(W_{t^*},G)\big)\geq\\
     \frac{\eta\epsilon^2(1-\epsilon)}{4} \sum_{t^*=0}^{\infty}  t^*\mathbb P(t^*)=     \frac{\eta\epsilon^2(1-\epsilon)}{4}\mathbb E[t^*].
\end{align*}
Since loss is non-negative
\[ \frac{4}{\eta\epsilon^2(1-\epsilon)}\mathbb E_{t^*} \mathbf{E}_{\mu}\big( \loss(W_{0},G)\big)\geq  \mathbb E[t^*] .\]
\end{proof}


==> importance_sampling.tex <==
\section{Theorem}

Next, we turn our attention to models, such as GraphSAINT \cite{zeng2019graphsaint}, that do not use SGD in estimating gradients  and instead, they use a more stylized probability distribution for the gradient sampler $\mu_g$.
We bound the number of training steps based on how far $\nu_g$ is from uniform sampling.  
This is quantified by the KL-divergence, which is a measure of the relative entropy between two distributions. For two given distributions $\rho$ and $\theta$, the relative entropy or KL-divergence is defined as $D_{KL}(\rho\mid\mid \theta)=\mathbb E_{x\sim \rho}\left(\log(\rho(x)/\theta(x))\right)$.  We use the result of \cite{chatterjee2018sample} to bound the sample size required in each minibatch to have a good estimation of the gradient. 

\begin{theorem}\label{thm: stochastic GNN importance sampling}
Consider a sampling-based GNN as in Algorithm~\ref{alg: training}, satisfying Assumptions ~\ref{assum: lipschitz}- \ref{assum: local}, and a subgraph sampler $\mu_S$ generating  convergent graphs $\{G_n\}_{n\in\mathbb N}$ as in Assumption \ref{assum: GL}.
Then, there exists a learning rate $\eta>0$ such that for any $\epsilon>0$, training Algorithm~\ref{alg: training} on the sequence $\{G_n\}_{n\in\mathbb N}$ converges to the $\epsilon$-neighborhood of the GNN learned on the limit, provided that $|V(G_n)|\geq N_\epsilon$ for some $N_\epsilon$. Further, the number of steps depends on the KL-divergence of $\nu_g$ and uniform sampling $U$, i.e.,  $\smash{\mathbb{E}_\mu[t^*]=O\big(\frac{\exp{D_{KL}(\nu_g|| U)}}{\eta\epsilon^2}\big)}$.
\end{theorem}

\section{Example}

\todo{go back here}
\noindent\textbf{GraphSAINT:}
GraphSAINT \cite{zeng2019graphsaint} offers an alternative approach to the scalability of GNNs by first sampling subgraphs and then training a full GNN on them. GraphSAINT employs various graph sampling techniques to define $\nu_C$, including random walk sampling, node sampling, and random edge sampling. Additionally, GraphSAINT proposes loss normalization to eliminate sample bias. Specifically, if $p_v$ is the probability of sampling a node, then the loss under GraphSAINT is given by
\[    \mathcal L'=\frac{1}{|\mathcal Y|}\sum_{v\in\mathcal Y}\frac{1}{|n|p_v}\mathcal L (\mathbf z_v(\mu_q(v))).\]
In terms of the framework of Algorithm~\ref{alg: training}, the gradient sampler is $\nu_g(v)=p_v$. 

\section{Gradient Estimation with Importance Sampling}\label{appendix: importance sampling}


% Next, we extend this result to GCNs with sampling, such as FastGCN and GraphSage and other paradigms described in Section~\ref{}. We show that under some assumptions, we can train these stochastic GCNs on large-enough graphs, and we these training framework converges  to a limit that could be described in two way: 1) the full GCN on a perturbation of the graph limit (the perturbation depends on sampling algorithms $\nu_C, \nu_g$, 2) or the stochastic GCN (e.g., GraphSage) on the actual graph limit.  This provides a theoretical foundation for understanding the convergence of GCNs with sampling, and has significant implications for the scalability and generalization of GCNs. 


% One of the advantages of using graph limits is that it allows us to have intuition about the limiting structure of the graph. In some cases, we can even obtain approximate learning coefficients directly from the limit. Furthermore, we can sample nodes from the limit with constant layers, which reduces the computational cost of gradient computation. This approach provides a good approximation of the full GCN model, without the need to train on the whole graph.


% First, we look at full-GCN when it is trained at each epoch on  large-enough samples of graphs with from the same family. We show that trainign GCN on these sampled graph, converges to  training GCN on the limit. Why we do this? 1- this is a new way of training for sparse graphs, start from a moderate scale graph and add nodes in each epoch.
% 2- Because sometimes we have intuition about the limiting structure, and we can get approximate learning coefficients from the limit directly. 
% 3- We can sample nodes from the limit with K layers of neighborhood. So, we don't have to find gradient on the whole graph, and gradient on these sampled nodes are a good approximation of the actual learning.

% This first set of results leads us to a more interesting direction as well. Consider the sampling method in GraphSage procedure. It can be applied to a graph family with limits as well and it gives us a new limit. Then all of above theorems  applies to this idea. We can train FastGCN on large enough graphs and it converges to GCN on the percolated graph limit or FastGCN on graph limit in a few steps $O(1/\epsilon^2)$ and the number of layers is 





% - Lemma 3.4 still holds (if we compute full gradient and not SGD), since the new function is still local.

% - Evaluating loss (in SGD): instead of actual gradient we sample nodes and evaluate the gradient. the number of sufficient samples depends on the limit. What about normalized sampling? (in lemma 3.4 we will then need minimum number of samples for SGD)


% A different version of Lemma 3.4.
% Use importance sampling? (If I can assume loss function is bounded from above)

Algorithm~\ref{alg: training} estimates the loss gradient $\nabla\mathcal L$ using the sampling scheme $\nu_g$. Let $\mathcal{Y}_B$ be the minibatch sampled by $\nu_g$. Then the sampling gradient $\nabla\tilde{\mathcal L}$ is defined as
\begin{equation}\label{eq: loss estimate weighted}
    \nabla\tilde{\mathcal L}_{\nu_g}(W_t,G_n)=\frac{1}{|\mathcal{Y}_B|}\sum_{v\in \mathcal{Y}_B}\frac{1}{\nu_g(v)} \nabla \loss(y_v,z_v).
\end{equation}
In some other architectures such GraphSage, this normalization is not done
\begin{equation}\label{eq: loss estimate unweighted}
    \nabla{\mathcal L}_{\nu_g}(W_t,G_n)=\frac{1}{|\mathcal{Y}_B|}\sum_{v\in \mathcal{Y}_B} \nabla \loss(y_v,z_v),
\end{equation}
where in these architectures, the sampling gradient does not converge to the actual gradient $\nabla\mathcal L$ \footnote{For example, in the presence of nonlinearities, GraphSAGE is biased.}. Instead, we show the sampling gradient converges to a similar sampling gradient defined on the limit. To formalize this idea, we need the sampling schemes $\nu_g$ and $\nu_C$ to be a function of the local neighborhood of the vertex $o$.
% \begin{assumption}[Local Samplers] \label{assum: local}The gradient sampling scheme $\nu_g$ and the computational graph sampling scheme $\nu_C$ are local (or $k$-local)  if there exists a constant $k$ independent from the size of the graph $G$, such that $\nu_g(v)$ for any vertex $v$ and $\nu_C(v)$ depend only on the $k$-ball neighborhood of $v$, $B_k(G,v)$.  
% \end{assumption}
% In above definition, a convenient choice for $k$ would be the number of layers in GCN. 
% In order to state our theorem, we require an additional assumption on the sampling schemes. Given a graph $G$, let $\Delta(G)$ denote its maximum degree. The assumption is that the $k$-local sampler, which depends on the $k$-neighborhoods, assigns a small probability to nodes with unbounded maximum degree in their $k$-neighborhood. 
\begin{assumption}[Uniformly Integrable Samplers] \label{assum: finite sampler} The $k$-local gradient sampling scheme $\nu_g$ and the computational graph sampling scheme $\nu_C$ are said to be uniformly integrable if for any $\epsilon>0$, there exists a constant $M_\epsilon$ , $N_\epsilon$ such that for $n>N_\epsilon$:
\[\sum_{v:\Delta(B_k(G_n,v))\geq M_\epsilon}\nu(v) \leq \epsilon n.\]
This means that the probability of sampling from subgraphs with a maximum degree larger than $M$ is bounded above by $\epsilon$.
\end{assumption}
% \begin{remark}
%  In many of the architectures discussed in Section~\ref{sec: }, $\nu_g$ is uniform sampling which satisfies both of the above assumptions on convergent graphs.
% % In many of the architectures discussed in Section~\ref{sec: }, $\nu_g$ is either the uniform sampling or it is proportional to the normalized adjacency matrix. The former sampling scheme always satisfies the uniform integrablity assumption on convergent graphs, and the latter sampling scheme satisfies the above assumption when the second moment of the degree sequence is uniformly integrable. 
% \end{remark}
% % Now, we can define the reweighted limit $\mu_s$. To construct $\mu_s$, first sample $(G,o)$ according to the limit $\mu$, and then accept this sample with probability $\nu_g(o)$. Now, draw the $k$ neighborhood of $o$ according to $\nu_C(o)$. 
% Now, we can state the main theorem.

% \begin{theorem}\label{thm: stochastic GCN}
% Given the assumptions of Theorem~\ref{thm: GCN} and local finite samplers $\nu_C$ and $\nu_g$ (Assumptions~\ref{assum: local} and \ref{assum: finite sampler}),
% then, there exists a small enough learning rate $\eta$ such that for any $\epsilon>0$, training stochastic GCN as in Algorithm~\ref{alg: training} with a constant number of layers (Assumption~\ref{assum: layers}) and Lipschitz loss function (Assumption~\ref{assum: lipschitz}) on the sequence of convergent graphs with learning rate $\eta$ converges to the $\epsilon$-neighborhood of training stochastic GCN in the limit in $\tilde O(\frac{1}{\epsilon^2})$ expected steps. Formally, if we define $t^*=\inf_t\{\mathbb{E}_{\mu,W_t}(\nabla \loss(W_t,G))\leq \epsilon\}$ then $\mathbb{E}_\mu[t^*]=O(\frac{1}{\eta\epsilon^2})$.
% \end{theorem}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

